JCoffee: Using Compiler Feedback to Make Partial Code Snippets Compilable

Static program analysis tools are often required to work with only a small part of a program's source code, either due to the unavailability of the entire program or the lack of need to analyze the complete code. This makes it challenging to use static analysis tools that require a complete and typed intermediate representation (IR). We present JCoffee, a tool that leverages compiler feedback to convert partial Java programs into their compilable counterparts by simulating the presence of missing surrounding code. It works with any well-typed code snippet (class, function, or even an unenclosed group of statements) while making minimal changes to the input code fragment. A demo of the tool is available here: https://youtu.be/O4h2g_n2Qls

==> table_errors_fixes.tex <==
\begin{table*}[t]
  \centering
  \caption{Most commonly encountered errors and their fixes.}
  \def\arraystretch{1.5}%  1 is the default
  \begin{tabular}{|p{0.33\linewidth}|p{0.3\linewidth}|p{0.3\linewidth}|}
    \hline
     \multicolumn{1}{|c|}{Sample Error} & \multicolumn{1}{c|}{Example} & \multicolumn{1}{c|}{Fix} \\ 
     \hline
      incompatible types: \code{UNKNOWN} cannot be converted to \code{URL} 
      & \code{URL url = H.getURL("abcd");} 
      & set the return type of \code{H.getURL(String)} function to \code{URL} \\
     \hline

      bad operand types for binary operator \code{$\geq$}
        \newline first type:  \code{UNKNOWN}, second type: \code{int}
      & \code{if (values[i] $\geq$ 0)} 
      & set the datatype of operand having \code{UNKNOWN} to \code{int} \\
     \hline

      incomparable types: \code{UNKNOWN} and \code{int} 
      & \code{if(resp.getCode() $\neq$ 304)} 
      & set the datatype of operand having \code{UNKNOWN} to \code{int} \\
     \hline

      invalid method declaration; return type required 
      & \code{public URL(String name)\{...\}} 
      & the code snippet was a constructor. Set return type to \code{void} in signature \\
     \hline

      no suitable method found for \code{add(BasicPair)}
       \newline method \code{Alternative \#1} is not applicable
       \newline reason for non-applicability
       \newline \ldots
      & \code{Pairs.add(BasicPair("a", "b"));}
         \newline \newline method \code{add(Pair)} is not applicable
         \newline \code{BasicPair} cannot be converted to \code{Pair}
      & Add a new method to the corresponding class with \code{add(BasicPair)} signature \\
     \hline

    %  \multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{cannot find symbol}}}
     cannot find symbol: class \code{Name}
     & \code{def.setName(new Name("foo"));}
     & create new class \code{Name} \\
     \hline
     
     cannot find symbol: method \code{getParam(String)}
     & \code{String mName = getParam("data");}
     & create new method \code{getParam(String)} in container class \\
     \hline

     cannot find symbol: variable \code{page}
     & \code{def.setName(page.getModName());}
     & create new variable \code{page} of type \code{UNKNOWN} \\ 
     \hline

     cannot find symbol: method \code{setNode(ID)}
     \newline location: variable \code{id} of type \code{Node}
     & \code{id.setNode(assertionId);} 
     & create new method \code{setNode(ID)} in class \code{Node} \\ 
     \hline

% variable xyz of type ABC 

     cannot find symbol: variable \code{entityId}
       \newline location: class \code{classA}
     & \code{audience.setNode(entityId);}
     & create new member variable \code{entityId} in class \code{classA} \\
     \hline
  \end{tabular}
  \label{table_EFM}
\end{table*}
